Learning to Perform Local Rewriting for Combinatorial Optimization

Search-based methods for hard combinatorial optimization are often guided by heuristics. Tuning heuristics in various conditions and situations is often time-consuming. In this paper, we propose NeuRewriter that learns a policy to pick heuristics and rewrite the local components of the current solution to iteratively improve it until convergence. The policy factorizes into a region-picking and a rule-picking component, each parameterized by a neural network trained with actor-critic methods in reinforcement learning. NeuRewriter captures the general structure of combinatorial problems and shows strong performance in three versatile tasks: expression simplification, online job scheduling and vehicle routing problems. NeuRewriter outperforms the expression simplification component in Z3; outperforms DeepRM and Google OR-tools in online job scheduling; and outperforms recent neural baselines and Google OR-tools in vehicle routing problems.

==> deprecated.tex <==
\eat{
\subsection{k-SAT}

We randomly generate $k$-SAT problems using the same generator as~\citep{amizadeh2018learning,selsam2018learning}, and follow the same training setup as~\citep{amizadeh2018learning}. We compare with DG-DAGRNN~\citep{amizadeh2018learning} and NeuroSAT~\citep{selsam2018learning}, which are neural networks specially designed for SAT problems. On problems with $3-10$ variables, {\ours} can solve $99\%$ of them, which is significantly better than both DG-DAGRNN ($91\%$) and NeuroSAT ($92\%$). On problems with $20$ variables, {\ours} can solve $72\%$ of them, while both DG-DAGRNN and NeuroSAT achieve $69\%$. This demonstrates that with a simple ruleset, {\ours} can effectively learn heuristics to solve small-scale SAT problems. Due to space limit, we defer more discussion to
\ifapp
Appendix~\ref{app:sat}.
\else
\appref.
\fi}
